Building Code with Dynamic Staging

When creating a new domain-specific language (DSL) it is common to embed it as a part of a flexible host language, rather than creating it entirely from scratch. The semantics of an embedded DSL (EDSL) is either given directly as a set of functions (shallow embedding), or an AST is constructed that is later processed (deep embedding). Typically, the deep embedding is used when the EDSL specifies domain-specific optimizations (DSO) in a form of AST transformations. In this paper we show that deep embedding is not necessary to specify most optimizations. We define language semantics as action functions that are executed during parsing. These actions build incrementally a new, arbitrary complex program function. The EDSL designer is able to specify many aspects of the semantics as a runnable code, such as variable scoping rules, custom type checking, arbitrary control flow structures, or DSO. A sufficiently powerful staging mechanism helps assembling the code from different actions, as well as evaluate the semantics in arbitrarily many stages. In the end, we obtain code that is as efficient as one written by hand. We never create any object representation of the code. No external traversing algorithm is used to process the code. All program fragments are functions with their entire semantics embedded within the function bodies. This approach allows reusing the code between EDSL and the host language, as well as combining actions of many different EDSLs.

==> template/tikzshapes.tex <==
\makeatletter
%\tikzset{arc style/.initial={}}
\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
% compute corner of ?flipped page?
\pgf@xc=\pgf@xb \advance\pgf@xc by-10pt % this should be a parameter
\pgf@yc=\pgf@yb \advance\pgf@yc by-10pt
% construct main path
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
}
}
\makeatother

\tikzstyle{document}=[shape=document,draw,inner ysep=18pt]
